Composing Distributed Computations Through Task and Kernel Fusion

We introduce Diffuse, a system that dynamically performs task and kernel fusion in distributed, task-based runtime systems. The key component of Diffuse is an intermediate representation of distributed computation that enables the necessary analyses for the fusion of distributed tasks to be performed in a scalable manner. We pair task fusion with a JIT compiler to fuse together the kernels within fused tasks. We show empirically that Diffuse's intermediate representation is general enough to be a target for two real-world, task-based libraries (cuNumeric and Legate Sparse), letting Diffuse find optimization opportunities across function and library boundaries. Diffuse accelerates unmodified applications developed by composing task-based libraries by 1.86x on average (geo-mean), and by between 0.93x--10.7x on up to 128 GPUs. Diffuse also finds optimization opportunities missed by the original application developers, enabling high-level Python programs to match or exceed the performance of an explicitly parallel MPI library.

==> mlir-intro-fig.tex <==
\begin{figure}
\begin{subfigure}[b]{0.49\textwidth}
\begin{center}
\begin{tabular}{c}
\begin{lstlisting}[language=C++, basicstyle=\fontsize{6}{8}\ttfamily]
class Task {
  // Standard implementation.
  void gpu_variant(
    vector<pair<Store, Priv>> args, 
  );
  // Opt-in MLIR task body generator.
  mlir::func::FuncOp generator(
    vector<pair<StoreDesc, Priv>> args, 
  );
};
\end{lstlisting}
\end{tabular}
\end{center}
\caption{API to define a task visible to \name{}.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
\begin{center}
\begin{tabular}{c}
\begin{lstlisting}[basicstyle=\fontsize{6}{8}\ttfamily]
func.func @kernel(
  %a: memref<?xf64>,
  %b: memref<?xf64>,
  %c: memref<?xf64>) {
  %dim = memref.dim %c, 0
  affine.for %i = 0 to %dim {
    %0 = affine.load %a[%i]
    %1 = affine.load %b[%i]
    %2 = arith.addf %0, %1
    affine.store %2, %c[%i] }
}
\end{lstlisting}
\end{tabular}
\end{center}
\caption{MLIR generated for an element-wise addition.}   
\label{fig:elemwise-mlir-fragment}
\end{subfigure}
\caption{\name{} generator API and generated MLIR fragment.}
\label{fig:example-api-and-mlir}
\end{figure}

==> system-overview.tex <==
\begin{figure}


\definecolor{adaee4ed-88c8-5b21-a9e7-31316ebef86f}{RGB}{255, 179, 178}
\definecolor{f3551e38-74df-57e2-b793-83d7fe876c85}{RGB}{102,102,102}
\definecolor{0b71a967-1f15-55a5-9bb9-70efa7b4fc58}{RGB}{51, 51, 51}
\definecolor{5856d031-3da1-575c-834e-c77e9e438c62}{RGB}{162, 177, 195}
\definecolor{nv-green}{RGB}{118, 185, 0}
\definecolor{ours}{RGB}{162, 204, 255}
% \definecolor{offwhite}{RGB}{250,250,250}

\tikzstyle{512bdd77-c3aa-5669-a956-85f7a90c6fb4} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, font=\normalsize, color=0b71a967-1f15-55a5-9bb9-70efa7b4fc58, draw=f3551e38-74df-57e2-b793-83d7fe876c85, line width=1, fill=adaee4ed-88c8-5b21-a9e7-31316ebef86f]
\tikzstyle{linestyle} = [thick, draw=5856d031-3da1-575c-834e-c77e9e438c62, line width=2, ->, >=stealth]

\tikzstyle{nv-lib-box} = [rectangle, rounded corners, text centered, font=\scriptsize, color=0b71a967-1f15-55a5-9bb9-70efa7b4fc58, draw=f3551e38-74df-57e2-b793-83d7fe876c85, line width=1]% , fill=offwhite]
\tikzstyle{our-box} = [rectangle, rounded corners, text centered, font=\scriptsize, color=0b71a967-1f15-55a5-9bb9-70efa7b4fc58, draw=f3551e38-74df-57e2-b793-83d7fe876c85, line width=1, fill=ours]
\tikzstyle{empty-box} = [rectangle, rounded corners, text centered, font=\scriptsize, color=0b71a967-1f15-55a5-9bb9-70efa7b4fc58, draw=f3551e38-74df-57e2-b793-83d7fe876c85, line width=1]


\begin{tikzpicture}[scale=0.8, transform shape]
\node (cunumeric) [nv-lib-box, align=center] { \cunumeric{} \\ \cite{cunumeric}};
\node (legate-sparse) [nv-lib-box, align=center, below=of cunumeric] {Legate Sparse \\ \cite{legate-sparse}};

\node (ir) [our-box, below right= 0.10cm and 1cm of cunumeric, align=center] {\name{} IR \\  (\Cref{sec:ir})};

\draw [linestyle] (cunumeric) --  (ir);
\draw [linestyle] (legate-sparse) --  (ir);

\node (task-fusion) [our-box, above right = 0.50cm and 1.0 cm of ir, align=center] {Distributed Task Fusion \\ (\Cref{sec:dist-task-fusion})};

\node (fusion-optimizations) [our-box, below=0.50cm of task-fusion, align=center] {Fusion Optimizations \\ (\Cref{sec:fusion-optimizations})};

\node (kernel-fusion) [our-box, below=0.50cm of fusion-optimizations, align=center] {JIT Kernel Fusion \\ (\Cref{sec:kernel-fusion})};

\node (compiler-box) [empty-box, fit={(task-fusion) (fusion-optimizations) (kernel-fusion)}, label=below:{\scriptsize \name{} Dynamic Analyses}] {};

\draw [linestyle] (ir) --  (compiler-box);
\draw [linestyle] (task-fusion) -- (fusion-optimizations);
\draw [linestyle] (fusion-optimizations) -- (kernel-fusion);

\node (legion) [nv-lib-box, align=center, right = of compiler-box] {Legion Runtime \\ \cite{legion}};

\draw [linestyle] (compiler-box) -- (legion);

\end{tikzpicture}

\caption{System Overview of \name{}. Highlighted components indicate our contributions.}
\label{fig:overview}
\end{figure}

==> weak-scaling-graphs.tex <==
% \begin{figure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/scholes.pdf}
% \caption{Black-Scholes Option Pricing}
% \label{fig:black-scholes}
% \end{subfigure}
% %
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/jacobi.pdf}
% \caption{Jacobi Iteration}
% \label{fig:jacobi}
% \end{subfigure}


% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/cg.pdf}
% \caption{Conjugate Gradient (CG)}
% \label{fig:cg}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/cgs.pdf}
% \caption{Conjugate Gradient Squared (CGS)}
% \label{fig:cgs}
% \end{subfigure}

% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/bicgstab.pdf}
% \caption{BiConjugate Gradient Stabilized (BiCGSTAB)}
% \label{fig:bicgstab}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/gmg.pdf}
% \caption{Geometric Multi-Grid Solver}
% \label{fig:gmg}
% \end{subfigure}



% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/cfd.pdf}
% \caption{Computational Fluid Dynamics Simulation}
% \label{fig:cfd}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.85\textwidth]{figures/torchswe.pdf}
% \caption{TorchSWE (Shallow-Water Equation Solver)}
% \label{fig:torchswe}
% \end{subfigure}

% \caption{All weak scaling experiments.}
% \end{figure}


% \begin{figure*}

% \begin{subfigure}{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/scholes.pdf}
% \caption{Black-Scholes}
% \label{fig:black-scholes}
% \end{subfigure}
% %
% \begin{subfigure}{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/jacobi.pdf}
% \caption{Jacobi Iteration}
% \label{fig:jacobi}
% \end{subfigure}
% %
% \begin{subfigure}{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/cg.pdf}
% \caption{CG}
% \label{fig:cg}
% \end{subfigure}
% %
% \begin{subfigure}{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/bicgstab.pdf}
% \caption{BiCGSTAB}
% \label{fig:bicgstab}
% \end{subfigure}

% \begin{subfigure}[h]{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/cgs.pdf}
% \caption{CGS}
% \label{fig:cgs}
% \end{subfigure}
%
% \hfill
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/gmg.pdf}
% \caption{GMG}
% \label{fig:gmg}
% \end{subfigure}\hfill
% %
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/cfd.pdf}
% \caption{CFD}
% \label{fig:cfd}
% \end{subfigure}\hfill
% %
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figures/torchswe.pdf}
% \caption{TorchSWE}
% \label{fig:torchswe}
% \end{subfigure}\hfill
% \hfill

% \begin{subfigure}[h]{\linewidth}
% \centering
% \includegraphics[width=0.7\textwidth]{figures/scholes.pdf}
% \caption{Black-Scholes Option Pricing}
% \label{fig:black-scholes}
% \end{subfigure}
% %
% \begin{subfigure}[h]{\linewidth}
% \centering
% \includegraphics[width=0.7\textwidth]{figures/jacobi.pdf}
% \caption{Jacobi Iteration}
% \label{fig:jacobi}
% \end{subfigure}

% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.9\textwidth]{figures/cg.pdf}
% \caption{Conjugate Gradient (CG)}
% \label{fig:cg}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.9\textwidth]{figures/cgs.pdf}
% \caption{Conjugate Gradient Squared (CGS)}
% \label{fig:cgs}
% \end{subfigure}

% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.9\textwidth]{figures/bicgstab.pdf}
% \caption{BiConjugate Gradient Stabilized (BiCGSTAB)}
% \label{fig:bicgstab}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\textwidth}
% \centering
% \includegraphics[width=0.9\textwidth]{figures/gmg.pdf}
% \caption{Geometric Multi-Grid Solver (GMG)}
% \label{fig:gmg}
% \end{subfigure}


% \caption{Weak scaling results across all applications (higher is better).}
% \end{figure*}
